Experimenting with Emerging RISC-V Systems for Decentralised Machine Learning

Decentralised Machine Learning (DML) enables collaborative machine learning without centralised input data. Federated Learning (FL) and Edge Inference are examples of DML. While tools for DML (especially FL) are starting to flourish, many are not flexible and portable enough to experiment with novel processors (e.g., RISC-V), non-fully connected network topologies, and asynchronous collaboration schemes. We overcome these limitations via a domain-specific language allowing us to map DML schemes to an underlying middleware, i.e. the FastFlow parallel programming library. We experiment with it by generating different working DML schemes on x86-64 and ARM platforms and an emerging RISC-V one. We characterise the performance and energy efficiency of the presented schemes and systems. As a byproduct, we introduce a RISC-V porting of the PyTorch framework, the first publicly available to our knowledge.

==> Chapters/0_Rebuttal.tex <==
\section*{\centering Experimenting with Emerging RISC-V Systems for Decentralised Machine Learning}

\begin{center}
{\Large \color{gray} Response to the reviewers}
\end{center}

We thank all the reviewers for their constructive comments. We read them carefully and tried to address each one to the best of our ability.

{\bf Reviewer 1}: We thank the reviewer for his appreciation of our work, understanding of our major contributions, and acknowledgement of the effort we put into porting all the proposed software to the RISC-V platform.

\paragraph{Q1.1}  
{\color{gray} \textit{"[...] the CPU frequency should have being set to a common value to all three evaluated platforms (Intel, Ampere, and SiFive). It would also be valuable to present results where each system is used to its fullest."}}

\paragraph{A1.1} 
We run additional experiments using each system to its fullest potential (increasing the number of cores) using a three-node setup (master plus 2 workers). The results to train one FL round on the x86-64 platform are: ~493ms using 1 core, ~490ms using 2 cores, ~580ms using 4 cores, ~792ms using 10 cores, ~1136 using 20 cores, and ~1578ms using all 40 cores.
The computing time increase with increasing cores because we train a small model to account for the (significantly) lower speed of the RISC-V. In such a scenario, the increasing thread handling and synchronization overhead dominate the runtime. We obtained similar results on the ARM-v8 platform. We also tried to use a bigger model (Resnet18 trained on CIFAR10), but in that case, the training time on RISC-V was unacceptably long (more than a day for a single epoch, not even FL round).

\paragraph{Q1.2} 
 {\color{gray} \textit{“[...] the comparison of the proposed RISC-pb2l+Fastflow is only contrasted with existing/competing implementations on SiFive and only for a specific scenario -- master-worker with 4 workers. The authors could make a stronger point by also contrasting with existing/competing on the other platforms as well. Outperforming on SiFive might be due to immature software stack.”}}

\paragraph{A1.2} 
We repeated the comparison also on the x86-64 architecture, which is the most mature from a software stack perspective, which leads to the same observations as on the RISC-V platform. A training with OpenFL with one server and four workers on the MNIST dataset with the same conditions, hyper-parameters and data handling as our previously run experiments took ~59.12 seconds to complete. If we compare such a result with our system's one in the same configuration, which is ~23.56 seconds, we see that our implementation is about 1.5 times faster than OpenFL, even on a more mature platform with a more optimised software stack. We added this result to the paper.


{\bf Reviewer 2}: We are grateful to the reviewer for bringing out some of this work’s aspects that can be further improved. We corrected the typos in the paper and tried our best to address the reviewer’s observations/criticisms as follows.


\paragraph{Q2.1}
{\color{gray} \textit{“The paper is often filled with inaccuracies, especially in the Introduction, with strong statements and no justification for said statements. This ranges from basic statements such as Arm being an emerging architecture (in the embedded/edge space, it is the opposite), to statements about Python's performance (ignoring the common use of optimized libraries in ML, which drive the bulk of performance). Implications (Section 2.3) that traditional frameworks and models focusing on the goodness of the learnt model may be a limitation (due to section header) is inaccurate. That is the point of such models, as else, what is the value?”}}

\paragraph{A2.1} 
While ARM is widely spread in edge devices, it is not the same at the server level, hence the word emergent. To better reflect our focus, we changed the title and text using RISC-V as the sole emerging platform in the paper.
One of the article’s aims is to show that using a lower-level language, such as C/C++, allows the programmer to optimize computation performance better. As noted by the reviewer, even in ML Python applications, all heavy computations are delegated to underlying highly-optimized libraries not written in Python. Even so, the combination of high- and low-level code does not come for free. Using the MNIST benchmark from the official PyTorch examples repository, we trained a CNN using the C++ and Python PyTorch API to compare the execution time. Note that the python script and the C++ program train the same CNN architecture and only differ in the language and used API. The results averaged across 5 runs show that the C++ API (314.5s) is ~40\% faster than the Python API (442.8s). We added these results to the paper.
We omitted the learning metrics because these depend on the specific algorithms that train and  aggregate the models. The proposed FL platform aims at allowing experimentation with diverse FL system designs, which is an orthogonal aspect to the learning algorithms. Here we do not aim to compare different learning algorithms. Please note that while using a different communication topology, the two FL examples (master-worker and peer-to-peer) compute the same aggregated model, as demonstrated in Section 4.1. We updated the paper clarifying this aspect.

\paragraph{Q2.2}
{\color{gray} \textit{“Expecting the inference cost [...] to be about 1/3 of the cost of training [...] is inaccurate. What data is there to justify this? Has there been any consideration that the duration of each step may be different?”}}

\paragraph{A2.2}
This statement has been made to say that the inference process typically costs a fraction of the training process, thus arguing that it can be handled differently. We took the $\frac{1}{3}$ from the cited research works:\\
{\small [1] Robert Adolf, Saketh Rama, Brandon Reagen, Gu-Yeon Wei, and David Brooks. 2016. Fathom: Reference workloads for modern deep learning methods. In 2016 IEEE International Symposium on Workload Characterization (IISWC). IEEE, Providence, RI, USA, 1–10. https://doi.org/10.1109/IISWC.2016.7581275}\\
{\small [16] Shen Li, Yanli Zhao, Rohan Varma, Omkar Salpekar, Pieter Noordhuis, Teng Li, Adam Paszke, Jeff Smith, Brian Vaughan, Pritam Damania, and Soumith Chintala. 2020. Pytorch distributed: Experiences on accelerating data parallel training. arXiv preprint arXiv:2006.15704 (28 June 2020). https://doi.org/10.48550/ARXIV.2006.15704}\\
We clarify that the ratio can differ from case to case but that the exact values is not crucial for the discussion.

\paragraph{Q2.3}
{\color{gray} \textit{“What is unclear is what of this work is ISA specific (especially as they initially aim to address a domain specific language, which should be as far from ISA as possible). The overall premise of the paper is not clear, and perhaps the focus should just be on porting FL to RISC-V [...] why is the FL system description in a high-level modelling language necessary? [...] the chosen methodology seems to add complexity for no added value.“}}

\paragraph{A2.3}
This work is not ISA-specific. The work aims to rethink the usual FL abstraction stack so that different collaboration networks can be tested and implemented. Also, we were interested in widening the range of usable processors. We started from the point at which all the existing frameworks (to our knowledge) implement a fixed collaboration schema  (master-worker), and no public implementations of Pytorch on RISC-V were available (either distributed or centralized). High-level modelling (and RISC-pb2) enables us to describe different communication patterns and automatically derive a distributed FastFlow implementation, which (being a vanilla header-only library for modern C++) was already working on RISC-V, thus easing the work of porting the ML because we ported and used only the single-node version of Pytorch/libtorch. Incidentally, this approach produces faster code than optimized Python code (i.e. Python with C++ libraries) on supported platforms. 

\paragraph{Q2.4}
{\color{gray} \textit{“[...] the authors should acknowledge they are comparing completely different classes of platforms. First of all, the SiFive platform is not energy efficient (a positive) despite being new. It was designed with such a purpose in mind. Secondly, the Intel and Arm platforms are server-grade, whilst the SiFive platform is embedded. Different efficiency levels are expected, and a more representative comparison would have been to use embedded platforms in all cases.”}}

\paragraph{A2.4}
Unfortunately, we do not have clusters of low-power Intel and Arm systems. Indeed, the SiFive is still not a server-grade processor. Still, it is nowadays among the more server-like RISC-V implementations (running Linux, with a good software stack available, including a gcc10). Several companies are trying to tape out a high-performance RISC-V processor (also including a vector/SIMD unit), such as those participating in the EU Pilot project and in the European Processor Initiative (EPI). Monte Cimone is regarded as the first RISC-V-based HPC system in the world (or at least a minion HPC system), see \url{https://www.hpcwire.com/off-the-wire/e4-announces-the-risc-v-based-monte-cimone-cluster/}. In this sense, our work can be seen as a preliminary study also investigating the current state of the current RISC-V capabilities and is preparatory for future experimentation with expected server-grade RISC-V processors, such as the Ventana processor (\url{https://www.ventanamicro.com}). We were not expecting the SiFive to outperform the Intel and ARM processors, but we still thought that a comparison could be helpful to check the status of this technology.

\paragraph{Q2.5}
{\color{gray} \textit{“[...] the authors are surprised that the SiFive platform performs well in the case of YOLOv5 despite its lack of a vector unit. The authors should provide insights into the vector utilisation on the other platforms before making such statements. Perhaps, there is little vector utilisation, or perhaps other reasons lead to the performance results.”}}

\paragraph{A2.5}
On Intel, we  compiled and linked Pytorch/libtorch with mathematics libraries supporting SIMD units supporting vector operations. Specifically, we used one-MKL (part of oneAPI) to exploit AVX-512 extension. For ARM, we used ARM Performance Libraries (\url{https://developer.arm.com/Tools%20and%20Software/Arm%20Performance%20Libraries}). The Arm Neoverse N1 processor includes two 128-bit SIMD units per core (Add, Multiply, fused Multiply-add). 

\paragraph{Q2.6}
{\color{gray} \textit{“Lastly, there is no mention of the quality of the model trained using their custom topology. This is critical for ML.”}}

\paragraph{A2.6}
We chose the master-worker and the peer-to-peer structure because they are mathematically equivalent, meaning that they will calculate the same ML model if set with the same seed, thus yielding the same performance. We demonstrated this in the paper by means of the RISC-pb2l formal language. The model obtained by the two communication topologies is the same, achieving ~95\% of accuracy; furthermore, this research work does not focus on the ML performance but on the computational performance.


{\bf Reviewer 3}: We thank the reviewer for sharing his take on our work and appreciate his interest.

\paragraph{Q3.1}
{\color{gray} \textit{“[...] it is not clear of the choice of RISC-pb2I library compared to other available.”}}

\paragraph{A3.1}
We choose the RISC-pb2l formal language because it can be directly translated into FastFlow code. FastFlow is a header-only C++11/17 library allowing us to run it on various computational platforms, including RISC-V, with little added effort and benefits from an optimised runtime. Also, see A.2.3. Thanks for raising the issue; we now better motivate our choice in the paper.

\paragraph{Q3.2}
{\color{gray} \textit{“The evaluation methodology could be improved by adding more models -- maybe a large model such as DenseNet and comparing against another cross-silo federated learning such as TFF.”}}

\paragraph{A3.2}
We experimented with a few larger models, such as the ResNet18 on CIFAR10. Still, those experiments did not make it to the final paper due to their prohibitive execution times on the SiFive processor. This setup takes approximately one day for a single federated round, implying that a single experiment, like the others presented in the paper, would require 20 rounds * 5 epochs * ~24 hours * 5 repetitions = 500 days (expected) on the RISC-V processor, which makes the experiment unfeasible. We hope to conduct more experiments on server-grade RISC-V as soon as they are available. We modified the paper to take care of these observations.


==> Garbage/3_DSL.tex <==
\section{DSL/libreria}
\td{Marco: aggiungere idea generale}
\td{Marco: aggiungere target di compilazione FF}
\gm{Fornire una classificazione sommaria dei vari tipi di FL e verificare quali sono coperti dal nostro DSL}

The first step in creating our middleware for FL is designing a high-level interface modelling language; such an interface should be sufficiently abstract to allow for the modelling of a wide range of computations while still being sufficiently specific to be easily applicable in different contexts.
With this aim in mind, we adopted a slightly modified version of the RISC-pb$^2$l formal language, making it suitable to express distributed workloads along the parallel ones. The basic building block of RISC-pb$^2$l are reported in \ref{tab:risc};

\begin{table}[t]
\begin{tabular}{|l|l|}
\hline
Syntax & 
  Semantics \\ \hline
$\left(\left(f\right)\right)$ &
  \textbf{Seq wrapper} Wraps sequential code into a RISC-pb$^2$l “function”. \\ \hline
$\left(\left| f \right|\right)$ &
  \textbf{Par wrapper} Wraps any parallel code into a RISC-pb$^2$l “function”. \\ \hline
${\left[\left|\Delta\right|\right]}_n$ &
  \textbf{Parallel} Computes in parallel $n$ identical programs on $n$ input items producing $n$ output items. \\ \hline
$\Delta_1 \bullet \dots \bullet \Delta_n$ &
  \textbf{Pipe} Uses $n$ (possibly) different programs as stages to process the input data items and to obtain output data items. Program $i$ receives inputs from program $i-1$ and delivers results to $i+1$. \\ \hline
$\left(_g\vartriangleright \right)$ &
  \textbf{Reduce} Computes a single output item using an $l$ level ($l\ge1$) $k$-ary tree. Each node in the tree computes a (possibly commutative and associative) $k$-ary function $g$. \\ \hline
$(_f\vartriangleleft)$ &
  \textbf{Spread} Computes $n$ output items using an $l$ level ($l\ge1$) $k$-ary tree. Each node in the tree uses function $f$ to compute $k$ items out of the input data items. \\ \hline
$\vartriangleleft_{D-Pol}$ &
  \textbf{1-to-N} Sends data received on the input channel to one or more of the n output channels, according to policy $D-Pol$ with $D-Pol\in\left[Unicast(p),Broadcast,Scatter\right]$ where $p\in \left[RR,AUTO\right]$. $RR$ applies a round robin policy, $AUTO$ directs the input to the output where a request token has been received \\ \hline
$\vartriangleright_{G-Pol}$ &
  \textbf{N-to-1} Collects data from the $n$ input channels and delivers the collected items on the single output channel. Collection is performed according to policy $G-Pol$ with $G-Pol\in\left[Gather, Gatherall, Reduce\right]$. $Gatherall$ waits for an input from all the input channels and delivers a vector of items, de facto implementing a barrier. \\ \hline
$\overleftarrow{\left(\Delta\right)}_{cond}$ &
  \textbf{Feedback} Routes output data $y$ relative to the input data $x (y = (x))$ back to the input channel or drives them to the output channel according to the result of the evaluation of $Cond(x)$. May be used to route back $n$ outputs to $n$ input channels as well. \\ \hline
\end{tabular}
\caption{RISC-pb$^2$l building block exploited in this research work.}
\label{tab:risc}
\end{table}

Symbols used:
$P$ set of participating peers, possibly divided into workers $W$ and aggregator $A$ nodes or leaf $L$, combiner $C$ and root $R$ (control room) nodes.
$r$ number of rounds

Usecase tree:
\begin{strip}
\centering
    \begin{align}
        \left(\left(\text{init}\right)\right) \bullet 
        \overleftarrow{\biggl( 
        \left[\left|\left(\left|\text{test}\right|\right)\right|\right]^{W} \bullet
        \left[\left|\left(\left|\text{train}\right|\right)\right|\right]^{W} \bullet
        \vartriangleright_{\text{Gall}} \bullet
        \left(\left(\text{FedAvg}\right)\right) \bullet
        \vartriangleleft_{\text{Bcast}}
        \biggr)_{r} }
        \equiv
        \left(\left(\text{init}\right)\right) \bullet 
        \overleftarrow{\biggl( 
        \left[\left|\left(\left|\text{test}\right|\right) \bullet 
        \left(\left|\text{train}\right|\right) \right|\right]^{W} \bullet
        \left(_{\text{FedAvg}}\vartriangleright\right) \bullet
        \vartriangleleft_{\text{Bcast}}
        \biggr)_{r}}
    \end{align}
    \begin{align}
        \left[\left|\left(\left(\text{init}\right)\right)\right|\right]^{P} \bullet
        \overleftarrow{\biggl( 
        \left[\left|\left(\left|\text{test}\right|\right)\right|\right]^{P} \bullet
        \left[\left|\left(\left|\text{train}\right|\right)\right|\right]^{P} \bullet
        \left[\left|\vartriangleleft_{\text{Bcast}} \bullet 
        \vartriangleright_{\text{Gall}} \bullet 
        \left(\left(\text{FedAvg}\right)\right) \right|\right]^{P}
        \biggr)_{r}}
        \equiv
        \left[\left|\left(\left(\text{init}\right)\right)\right|\right]^{P} \bullet
        \overleftarrow{\biggl( 
        \left[\left|\left(\left|\text{test}\right|\right) \bullet 
        \left(\left|\text{train}\right|\right) \bullet
        \vartriangleleft_{\text{Bcast}} \bullet
        \left(_{\text{FedAvg}}\vartriangleright\right) \right|\right]^{P}
        \biggr)_{r}}
    \end{align}
    \begin{align}
        \left(\left(\text{init}\right)\right) \bullet
        \overleftarrow{\biggl( 
        \left[\left|\text{infer}\right|\right]^{L} \bullet 
        \left(_\mathcal{F} \vartriangleright\right) \bullet 
        \left[\left|\text{combine}\right|\right]^{C} \bullet 
        \left(_\mathcal{F} \vartriangleright \right) \bullet 
        \left(\left(\text{alert}\right)\right)^{R} 
        \biggr)_{\infty}} \\
    \end{align}
\end{strip}

Usecase P2P:


Usecase distributed inference:


Usecase cyclic incremental learning (WIP):
\[
((\text{init})) \bullet
\overleftarrow{
\left(
(|\text{train}_1|) \bullet
\dots \bullet
(|\text{train}_i|) \bullet
\dots \bullet
(|\text{train}_{n_w}|)
\right)
}_{r}
\]

% \begin{figure}
%     \centering
%     \lstinputlisting[language=python, label=lst:exampleGraphs, caption={}, captionpos=b]{Figures/ff-example/exampleGraphs.py}
% \end{figure}

%\begin{figure}
%    \centering
%    \lstinputlisting[language=yaml, label=lst:exampleGraphs, caption={}, %captionpos=b]{Figures/ff-example/exampleGraphs_v2.yml}
%\end{figure}

% deadline Lunedi 17
% percentuale di ingaggio 
% persona di riferimento


% FL1
% M4 difficolta nel valutare afidabilita e consumi di riscv in ambito HPC


% FL2
% M4 survey on acceleratori e tool da usare

% due slides con gli interessi e skills per match making


==> Garbage/3_DSL_old.tex <==
\section{DSL/libreria}

The first step in the creation of a flexible and efficient middleware is the design of a domain-specific language capable of describing different FL processes from a high-level perspective.
We thus propose a Domain-Specific Language (DSL) for the FL scenario made up 
\td{Marco: aggiungere idea generale}
\td{Marco: aggiungere target di compilazione FF}
\gm{Fornire una classificazione sommaria dei vari tipi di FL e verificare quali sono coperti dal nostro DSL}

Symbols used:
$n_w$ number of workers  
$r$ number of rounds

Usecase tree:
\begin{strip}
\centering
    \begin{align}
        \left(\left(\text{init}\right)\right) \bullet 
        \overleftarrow{\left( 
        \left[\left|\left(\left|\text{train}_1\right|\right), ..., \left(\left|\text{train}_{n_w}\right|\right)\right|\right] \bullet
        \vartriangleright_{\text{Gatherall}} \bullet
        \left(\left(\text{FedAvg}\right)\right) \bullet
        \vartriangleleft_{\text{Broadcast}} \bullet
        %\left[\left|\left(\left|\text{train}\right|\right)\right|\right]_{n_w} \bullet
        %\left(_{\text{fedavg}}\vartriangleright\right) \bullet 
        %\left(\left|\text{test}\right|\right) \;  
        [|(|\text{test}_1|), ..., (|\text{test}_{n_w}|)|]
        \right) }_{r} \\
        \equiv
        \left(\left(\text{init}\right)\right) \bullet 
        \overleftarrow{\left( 
        \left[\left|\left(\left|\text{train}_1\right|\right), ..., \left(\left|\text{train}_{n_w}\right|\right)\right|\right] \bullet
        \left(_{\text{FedAvg}}\vartriangleright\right) \bullet
        \vartriangleleft_{\text{Broadcast}} \bullet
        \left[\left|\left(\left|\text{test}_1\right|\right), ..., \left(\left|\text{test}_{n_w}\right|\right)\right|\right]
        \right)}_{r}
    \end{align}
    \begin{align}
        \left[\left(\left(\text{init}\right]\right]\right]_{n_w} \bullet
        \overleftarrow{\left( 
        %\left[|
        %(|\text{train}|) \bullet
        \left[\left|\left(\left|\text{train}_1\right|\right], ..., \left(\left|\text{train}_{n_w}\right|\right]\right|\right] \bullet
        %\vartriangleleft_{\text{Broadcast}} \bullet
        \left[\left| \vartriangleleft_{\text{Broadcast}} \bullet 
        \vartriangleright_{\text{Gatherall}} \bullet 
        \left(\left(FedAvg\right]\right] \right|\right]_{n_w} \bullet
        %(_{\text{fedavg}}\vartriangleright) \bullet 
        %(|\text{test}|)
        \left[\left|\left(\left|\text{test}_1\right|\right], ..., \left(\left|\text{test}_{n_w}\right|\right]\right|\right]
        %|\right]_{n_w}
        \right)}_{r} \\
        \equiv
        \left[\left(\left(\text{init}\right]\right]\right]_{n_w} \bullet
        \overleftarrow{\left( 
        \left[\left|\left(\left|\text{train}_1\right|\right], ..., \left(\left|\text{train}_{n_w}\right|\right]\right|\right] \bullet
        \left[\left| \vartriangleleft_{\text{Broadcast}} \bullet
        \left(_{\text{FedAvg}}\vartriangleright\right] \right|\right]_{n_w} \bullet 
        \left[\left|\left(\left|\text{test}_1\right|\right], ..., \left(\left|\text{test}_{n_w}\right|\right]\right|\right]
        \right]}_{r}
    \end{align}
    \begin{align}
        ((\text{init})) \bullet
        \overleftarrow{\left( [|\text{infer}|]_{n_w} \bullet (_\mathcal{F} \vartriangleright) \bullet [|\text{combine}|]_{n_{w'}} \bullet (_\mathcal{F} \vartriangleright) \bullet ((\text{alert})) \right)}_{\infty} \\
    \end{align}
\end{strip}

Usecase P2P:


Usecase distributed inference:


Usecase cyclic incremental learning (WIP):
\[
((\text{init})) \bullet
\overleftarrow{
\left(
(|\text{train}_1|) \bullet
\dots \bullet
(|\text{train}_i|) \bullet
\dots \bullet
(|\text{train}_{n_w}|)
\right)
}_{r}
\]

% \begin{figure}
%     \centering
%     \lstinputlisting[language=python, label=lst:exampleGraphs, caption={}, captionpos=b]{Figures/ff-example/exampleGraphs.py}
% \end{figure}

\begin{figure}
    \centering
    \lstinputlisting[language=yaml, label=lst:exampleGraphs, caption={}, captionpos=b]{Figures/ff-example/exampleGraphs_v2.yml}
\end{figure}

% deadline Lunedi 17
% percentuale di ingaggio 
% persona di riferimento


% FL1
% M4 difficolta nel valutare afidabilita e consumi di riscv in ambito HPC


% FL2
% M4 survey on acceleratori e tool da usare

% due slides con gli interessi e skills per match making

